Comment on Revisiting Neural Program Smoothing for Fuzzing

MLFuzz, a work accepted at ACM FSE 2023, revisits the performance of a machine learning-based fuzzer, NEUZZ. We demonstrate that its main conclusion is entirely wrong due to several fatal bugs in the implementation and wrong evaluation setups, including an initialization bug in persistent mode, a program crash, an error in training dataset collection, and a mistake in fuzzing result collection. Additionally, MLFuzz uses noisy training datasets without sufficient data cleaning and preprocessing, which contributes to a drastic performance drop in NEUZZ. We address these issues and provide a corrected implementation and evaluation setup, showing that NEUZZ consistently performs well over AFL on the FuzzBench dataset. Finally, we reflect on the evaluation methods used in MLFuzz and offer practical advice on fair and scientific fuzzing evaluations.

==> evidence.tex <==
\section{Evidential Fallacy}
The main conclusion of MLFuzz is actually an evidential fallacy that lacks sufficient experimental evidence. MLFuzz claims that the performance of NEUZZ does not hold. This strong argument does not specify a particular set of programs, indicating that the performance of NEUZZ does not hold on any programs. To support such an argument, the authors have to show the evaluation result of NEUZZ on diverse sets of programs. However, we find that MLFuzz only evaluates a single dataset--the FuzzBench programs with which NEUZZ is \underline{\emph{incompatible}}. Although the set of programs and artifacts used in the NEUZZ paper have been open-sourced on GitHub, MLFuzz chooses to ignore them without any justification. Note that the FuzzBench dataset was released in 2020, two years after the publication of NEUZZ. Therefore, MLFuzz's main conclusion cannot be supported by their biased evaluation. In the next section, we explain several fatal implementation bugs in their biased evaluation, leading to unexpected fuzzer crashes and invalid experimental results. 


